Task-Driven Data Verification via Gradient Descent

We introduce a novel algorithm for the detection of possible sample corruption such as mislabeled samples in a training dataset given a small clean validation set. We use a set of inclusion variables which determine whether or not any element of the noisy training set should be included in the training of a network. We compute these inclusion variables by optimizing the performance of the network on the clean validation set via "gradient descent on gradient descent" based learning. The inclusion variables as well as the network trained in such a way form the basis of our methods, which we call Corruption Detection via Gradient Descent (CDGD). This algorithm can be applied to any supervised machine learning task and is not limited to classification problems. We provide a quantitative comparison of these methods on synthetic and real world datasets.

==> ML-verify.tex <==
\begin{figure}[ht]
		\centering
		\begin{tikzpicture}
		\node[det, shape=rectangle, scale=0.8] (DC) {\;Data Collection \;};
		\node[det, shape=rectangle, scale=0.8, below=0.5cm of DC] (verify1) {\;Manual Verification\;};
		\node[det, shape=rectangle, scale=0.8, right=0.5cm of DC] (model) {\;Model Building\;};
		\node[det, shape=rectangle, scale=0.8, below=0.5cm of verify1, xshift=2cm] (verify2) {\;ML Verification\;};
		\node[det, shape=rectangle, scale=0.8, below=0.5cm of verify2] (train) {\;Training \& Analysis\;};
		
		\path[-Stealth]
		(DC) edge (verify1)
		(verify1) edge (verify2)
		(model) edge (verify2)
		(verify2) edge (train);
		
        \draw [-Stealth] (verify2.west)  .. controls (-1,-1.7)  and (-2,-1.3) .. (verify1.west);
        \draw [-Stealth] (train.east)  .. controls (3.5,-2.1)  and (4.3,-0.4) .. (model.east);
		
		\end{tikzpicture}\caption{Data analysis work-flow with task based sample verification.}
		\label{fig:workflow}
	\end{figure}

==> no-verify.tex <==
	\begin{figure}[ht]
		\centering
		\begin{tikzpicture}
		\node[det, shape=rectangle, scale=0.8] (DC) {\;Data Collection \;};
		\node[det, shape=rectangle, scale=0.8, below=0.5cm of DC] (verify1) {\;Manual Verification\;};
		\node[det, shape=rectangle, scale=0.8, right=0.5cm of DC] (model) {\;Model Building\;};
		\node[det, shape=rectangle, scale=0.8, below=0.5cm of verify1, xshift=2cm] (train) {\;Training \& Analysis\;};
		
		\path[-Stealth]
		(DC) edge (verify1)
		(verify1) edge (train)
		(model) edge (train);
		
        \draw [-Stealth] (train.east)  .. controls (3.5,-2.1)  and (4.3,-0.4) .. (model.east);
		
		\end{tikzpicture}\caption{Data analysis work-flow.}
		\label{fig:man-verify}
	\end{figure}
